Discrete Empirical Interpolation Method for nonlinear softening problems involving damage and plasticity

Accurate simulations are essential for engineering applications, and intricate continuum mechanical material models are constructed to achieve this goal. However, the increasing complexity of the material models and geometrical properties lead to a significant increase in computational effort. Model order reduction aims to implement efficient methods for accelerating the simulation process while preserving a high degree of accuracy. Numerous studies have already demonstrated the benefits of this method for linear elastic material modeling. However, in the present work, we investigate a two-surface gradient-extended damage-plasticity model. We conducted complex simulations with this model, demonstrating both damage behavior and softening. The POD-based discrete empirical interpolation method (DEIM) is introduced and implemented. To accomplish simulations with DEIM and softening behaviour, we propose the implementation of a reduced form of the arc-length method. Existing research on calculating models with both damage and softening behavior using the DEIM and arc-length method is limited. To validate the methods, two numerical examples are thoroughly investigated in this study: a plate with a hole and an asymmetrically notched specimen. The results show that the proposed methods can create a reduced order model with high accuracy and a significant speedup of the simulation. For both examples, the analysis is conducted in three steps: first, plasticity without damage is examined, followed by damage without plasticity, and finally, the combination of plasticity and damage is investigated.

==> Chapter/0_abstract.tex <==
\section{Abstract}

Accurate simulations are essential for engineering applications, and intricate continuum mechanical material models are constructed to achieve this goal. 
However, the increasing complexity of the material models and geometrical properties lead to a significant increase in computational effort. 
Model order reduction aims to implement efficient methods for accelerating the simulation process while preserving a high degree of accuracy.
Numerous studies have already demonstrated the benefits of this method for linear elastic material modeling.
However, in the present work, we investigate a two-surface gradient-extended damage-plasticity model.
We conducted complex simulations with this model, demonstrating both damage behavior and softening.
The POD-based discrete empirical interpolation method (DEIM) is introduced and implemented. 
To accomplish simulations with DEIM and softening behaviour, we propose the implementation of a reduced form of the arc-length method.
Existing research on calculating models with both damage and softening behavior using the DEIM and arc-length method is limited.
To validate the methods, two numerical examples are thoroughly investigated in this study: a plate with a hole and an asymmetrically notched specimen. 
The results show that the proposed methods can create a reduced order model with high accuracy and a significant speedup of the simulation. 
For both examples, the analysis is conducted in three steps: first, plasticity without damage is examined, followed by damage without plasticity, and finally, the combination of plasticity and damage is investigated.

==> Chapter/2_Material_model.tex <==
\section{Material Model}
\label{sec:mat}

In the following section, the constitutive model used to investigate the proposed model order reduction approach will be briefly introduced. The material model was developed by Brepols et al. \cite{brepols2020} and serves as the finite strain version of the small strain version of the model \cite{brepols2017}. In principle, the material model is based on the micromorphic approach proposed by Forest \cite{forest2009}. The approach of Forest can be seen as a systematic approach to construct high-level gradient material models of already existing 'local' counterparts. The model introduces an additional nodal degree of freedom for the micromorphic damage. The Helmholtz free energy depends on the difference between the global damage and the local damage which can be strongly coupled by a penalty parameter. This approach is chosen to overcome a general problem of conventional continuum mechanical local damage models, where the softening regime is highly dependent on the mesh discretization in a finite element simulation.

Because the model is implemented with finite deformation kinematics, the reference configuration $B_0$ at time $t_0$ and the current configuration $B_t$ at time $t$ of a body are differentiated. For the different configurations, the position of a material point is described by the vectors $\bm{X}$ and $\bm{x}$, respectively. The current position of a material point can be obtained by adding a displacement vector $\buu$ to the position of the material point in reference configuration such that $\bm{x} = \bm{X} + \buu$. Assuming there exists a mapping $\bm{x} = \bChi(\bm{X}, t)$, the deformation gradient can be introduced as $\bF \coloneqq \partial \bChi(\bm{X},t)/\partial \bm{X}$. To model elastoplastic material behavior, the deformation gradient is multiplicatively decomposed into the elastic part $\bF_e$ and the plastic part $\bF_p$. Because the model includes Armstrong-Frederick type non-linear kinematic hardening, the plastic part of the deformation gradient is further decomposed into the recoverable part $\bF_{p_e}$ and the irrecoverable part $\bF_{p_i}$. After these splits, the deformation gradient reads
\be
\bF = \bF_e \bF_p \text{~ with ~} \bF_p = \bF_{p_e} \bF_{p_i}
\ee
and from this, the elastic Cauchy-Green deformation tensors are derived as
\be
\bC_e = \bF_e\T \bF_e, \qquad \bC_{p_e} = \bF_{p_e} \T \bF_{p_e}.
\ee
Having defined these tensors, the Helmholtz free energy is assumed to be
\be
\psi = f_{\textrm{dam}}(D)(\psi_e(\bC_e)+\psi_p(\bC_{p_e}, \xi_p))+\psi_d(\xi_d) + \psi_{\bar{d}}(D-\Dbar, \Grad(\Dbar))
\ee
where $\psi_e$ and $\psi_p$ denote the elastic and plastic part of the free energy, respectively. In addition to the recoverable plastic part of the Cauchy-Green deformation tensor, the plastic part of the free energy also depends on the accumulated plastic strain $\xi_p$. The energy related to damage hardening is stored in $\psi_d$ and the energy related to the micromorphic extension is stored in $\psi_{\bar{d}}$. Furthermore, the damage hardening energy is dependent on the accumulated damage $\xi_d$ and the energy related to the micromorphic extension is dependent on the micromorphic damage variable $\Dbar$. Lastly, the scalar-valued weakening function $f_{\textrm{dam}}(D)$ is introduced. The elastic energy is chosen as a compressible Neo-Hookean type and reads
\be
\psi_e = \dfrac{\mu}{2}\left(\tr \bC_e - 3 - 2\ln\left(\sqrt{\det\bC_e}\right)\right) + \dfrac{\lambda}{4}\left(\det\bC_e -1 -2 \ln\left(\sqrt{\det\bC_e}\right)\right)
\ee
with the two Lamé constants $\mu$ and $\lambda$. The plastic energy is defined as
\be
\psi_p = \dfrac{a}{2}\left(\tr \bC_{p_e} - 3 - 2\ln\left(\sqrt{\det\bC_{p_e}}\right)\right) + e\left(\xi_p + \dfrac{\exp(-f \xi_p)-1}{f}\right).
\ee
The material parameters $a$, $e$ and $f$ are related to kinematic and non-linear Voce isotropic hardening, with another parameter $b$ showing up in the evolution equation of $\dot{\bC}_{p_i}$.
The energy related to Voce damage hardening is defined as
\be
\psi_d = r\left(\xi_d + \dfrac{\exp\left(-s\xi_d\right) - 1}{s} \right)
\ee
where $r$ and $s$ are the two damage hardening material parameters. The energy of the micromorphic extension reads
\be
\psi_{\bar{d}} = \dfrac{H}{2}(D-\Dbar)^2 + \dfrac{A}{2} \Grad(\Dbar)\cdot\Grad(\Dbar)
\ee
with the aforementioned penalty parameter $H$ and the parameter $A$. An internal length scale is introduced into the material as $L \coloneqq \sqrt{A / H}$ which can be understood as a localization limiter, preventing the aforementioned localization of damage into a zone of vanishing volume. Choosing the penalty parameter to be a very high number allows for a strong coupling between the micromorphic and the local damage variable. The constitutive equations with respect to the reference configuration are based on the Clausius-Duhem inequality in order to fulfill the second law of thermodynamics. The derivation of the constitutive equations is carefully described by Brepols et al. \cite{brepols2020} and because it is not the main topic of this thesis, only the resulting equations are given below:

$\bullet$ State laws:
\bea
\bS &= \fdam(D) \, 2 \, \bF_p\ME \dfrac{\partial \psi_e}{\partial \bC_e}\bF_p\MT\\
&= \fdam(D) \left(\mu \, (\bC_p\ME - \bC\ME) + \dfrac{\lambda}{2} \left(\dfrac{\det \bC}{\det \bC_p} - 1 \right) \bC\ME \right)
\eea
\be
a_{0_i} = \dfrac{\partial \psi_{\bar{d}}}{\partial \Dbar} = -H (D-\Dbar)
\label{eq:a}
\ee
\be
\bbbb_{0_i} = \dfrac{\partial \psi_{\bar{d}}}{\partial \Grad(\Dbar)} = A \, \Grad(\Dbar)
\label{eq:b}
\ee
$\bullet$ Thermodynamic conjugate forces - plasticity:
\be
\bX = \fdam(D) \, 2 \, \bF_{p_i}\ME \dfrac{\partial \psi_e}{\partial \bC_{p_e}}\bF_{p_i}\MT = \fdam(D)\,a\,(\bC_{p_i}\ME - \bC\ME)
\ee
\be
q_p = \fdam(D)\,\dfrac{\partial \psi_p}{\partial \xi_p} = \fdam(D)\,e\,(1 - \exp(-f\xi_p))
\ee
$\bullet$ Thermodynamic conjugate forces - damage:
\be
Y = - \dfrac{\dd \fdam(D)}{\dd D}\,(\psi_e+\psi_p)-\dfrac{\partial \psi_{\bar{d}}}{\partial D} = - \dfrac{\dd \fdam(D)}{\dd D}\,(\psi_e+\psi_p) - H(D-\Dbar)
\ee
\be
q_d = \dfrac{\partial \psi_d}{\partial \xi_d} = r\,(1 - \exp(-s \, \xi_d))
\ee
$\bullet$ Auxillary stress tensors:
\be
\bY = \bC \bS - \bC_p \bX, \quad \bY_{\textrm{kin}} = \bC_p \bX
\ee
$\bullet$ Evolution equations are expressed in terms of effective (i.e., 'undamaged') quantities:
\be
\tilde{(\bullet)} \coloneqq \frac{(\bullet)}{\fdam(D)}
\ee
\be
\dot{\bC}_p = 2 \, \dot{\lambda}_p \dfrac{\sqrt{3/2}}{\fdam(D)}\dfrac{\tilde{\bY}^{'} \bC_p}{\sqrt{\tilde{\bY}^{'} \cdot (\tilde{\bY}^{'})\T}}, \quad \dot{\bC}_{p_i} = 2 \, \dot{\lambda}_p \dfrac{b/a}{\fdam(D)} \bY^{'}_{\textrm{kin}} \bC_{p_i}
\ee
\be
\dot{\xi}_p = \dfrac{\dot{\lambda}_p}{\fdam(D)}, \quad \dot{D} = \dot{\lambda}_d, \quad \dot{\xi}_d = \dot{\lambda}_d
\ee
$\bullet$ Yield and damage loading function:
\be
\Phi_p = \sqrt{3/2} \sqrt{\tilde{\bY}^{'} \cdot (\tilde{\bY}^{'})\T} - (\sigma_0 + \tilde{q}_p), \quad \Phi_d = Y - (Y_0 + q_d)
\label{eq:threshold}
\ee
$\bullet$ Loading / unloading conditions
\bea
\dot{\lambda}_p \ge 0, \qquad \Phi_p \le 0, \qquad \dot{\lambda}_p \Phi_p = 0\\
\dot{\lambda}_d \ge 0, \qquad \Phi_d \le 0, \qquad \dot{\lambda}_d \Phi_d = 0
\eea
Adding the initial yield stress $\sigma_0$ and damage threshold $Y_0$ in equation \ref{eq:threshold}, the material model has twelve material parameters in total ($\lambda$, $\mu$, $\sigma_0$, $a$, $b$, $e$, $f$, $Y_0$, $r$, $s$, $A$, $H$) which should be optimally determined from experimental data. Finally, the micromorphic balance equation can be written as
\bea
H(D-\Dbar)+ A \, \Ddiv(\Grad(\Bar{D})) &= 0 \quad \text{in } B_0\\
\Grad(\Dbar) \cdot \bn_0 &= 0 \quad \text{on } \partial B_0
\eea
Having the micromorphic balance equation at hand as well as the balance of linear momentum
\bea
\Ddiv(\bF \bS) + \bff_0 &= 0 \quad &&\text{in } B_0 \\
\bF \bS[\bn_0] &= \bt_0 \quad &&\text{on } \partial B_0\\
\buu &= \hat{\buu} \quad &&\text{on } \partial B_0
\eea
the weak form of the problem can be constructed. This is done via the usual procedure: First, the balance equations are multiplied by the appropriate test functions $\delta \buu$ in case of the linear momentum and $\delta \Dbar$ in case of the micromorphic balance and then integrated over the reference domain $B_0$. After that partial integration and the divergence theorem are applied such that the weak form reads:
\be
g(\buu, \Dbar, \delta \buu) \coloneqq \int_{B_0} \bS \cdot \delta \bE \: \dd V - \int_{B_0} \bff_0 \cdot \delta \buu \: \dd V - \int_{\partial B_{0_t}} \bt_0 \cdot \delta \buu \: \dd A = 0 \quad \forall \delta \buu
\ee
\be
h(\buu, \Dbar, \delta \Dbar) \coloneqq \int_{B_0} (H(D- \Dbar)\delta \Dbar - A \, \Grad(\Dbar) \cdot \Grad(\delta \Dbar))\dd V = 0 \quad \forall \delta \Dbar
\ee
The weak form is generally nonlinear and therefore it has to be linearized with respect to the unknowns and iteratively solved. The mathematical details of the linearization can again be found in \cite{brepols2020}. The linearized weak form is given by
\be
\begin{gathered}
    \int_{B_0} \Grad(\delta \buu) \cdot(\Grad(\Delta \buu) \mathbf{S}) \mathrm{d} V+\int_{B_0} \delta \bE \cdot \frac{\partial \mathbf{S}}{\partial \bE}[\Delta \bE] \mathrm{d} V+\int_{B_0} \delta \bE \cdot \frac{\partial \mathbf{S}}{\partial D} \Delta \Dbar \mathrm{~d} V \\
    =-\left(\int_{B_0} \delta \bE \cdot \mathbf{S} \mathrm{d} V-\int_{B_0} \delta \buu \cdot \boldsymbol{f}_0 \mathrm{~d} V-\int_{\partial B_{0_1}} \delta \buu \cdot \boldsymbol{t}_0 \mathrm{~d} A\right) \quad \forall \delta \buu
\end{gathered}
\label{eq:linmomentum}
\ee
\be
\begin{gathered}
    \int_{B_0} \delta \bar{D} H \frac{\partial D}{\partial \mathbf{E}} \cdot \Delta \mathbf{E} \mathrm{d} V+\int_{B_0}\left(\delta \bar{D} H\left(\dfrac{\partial D}{\partial \bar{D}}-1\right) \Delta \bar{D}-\operatorname{Grad}(\delta \bar{D}) \cdot A \operatorname{Grad}(\Delta \bar{D})\right) \mathrm{d} V \\
    =-\int_{B_0}(\delta \bar{D} H(D-\bar{D})-\operatorname{Grad}(\delta \bar{D}) \cdot A \operatorname{Grad}(\bar{D})) \mathrm{d} V \quad \forall \delta \bar{D}
\end{gathered}
\label{eq:linmicromorphic}
\ee
where $\D \bE$ is defined as $\D \bE \coloneqq 1/2(\bF \T \Grad(\D \buu) + \Grad(\D \buu)\T \bF)$.

To arrive at a computationally solvable problem, the finite element approximation of the linearized weak form is introduced. The reference body $B_0$ is approximated by $n_{el}$ finite elements $B_0^e$ and therefore the geometry of a body is defined as
\be
B_0 \approx \bigcup_{e=1}^{n_{el}} B_0^e.
\ee
This means that the integrals over the whole domain in the linearized weak form can be approximated by the sums of the contributions of all individual elements. After this, the exact displacement field $\buu(\bX)$, the micromorphic damage field $\Dbar(\bX)$, as well as their respective test functions, are approximated by shape functions such that
\bea
\begin{array}{l l}
    \buu(\bm{X}) \approx \bN_u^e(\bm{X})\bm{u}^e \qquad        & \delta \buu(\bm{X}) \approx \bN_u^e(\bm{X}) \delta \bm{u}^e        \\
    \Dbar(\bm{X}) \approx \bN_{\Dbar}^e(\bm{X})\bDbar^e \qquad & \delta \Dbar(\bm{X}) \approx \bN_{\Dbar}^e(\bm{X}) \delta \bDbar^e
\end{array}
\qquad \bm{X} \in B_0^e
\label{eq:approxu}
\eea
where $\bm{u}^e$ describes the vector containing the nodal values of the displacements and $\bDbar^e$ denotes a vector containing the nodal values of the micromorphic damage of the element. $\bN_u^e$ and $\bN_{\Dbar}^e$ are the matrices with the corresponding shape functions of the element. Similarly to \ref{eq:approxu} the included gradients can be approximated by
\bea
\begin{array}{l l}
    \Grad(\buu(\bm{X})) \approx \bB_{0u}^e(\bm{X})\bm{u}^e \qquad      & \Grad(\delta \buu(\bm{X})) \approx \bB_{0u}^e(\bm{X}) \delta \bm{u}^e      \\
    \Grad(\Dbar(\bm{X})) \approx \bB_{0\Dbar}^e(\bm{X})\bDbar^e \qquad & \Grad(\delta \Dbar(\bm{X})) \approx \bB_{0\Dbar}^e(\bm{X}) \delta \bDbar^e
\end{array}
\qquad \bm{X} \in B_0^e
\label{eq:approxgrad}
\eea
with matrices $\bB_{0u}^e \coloneqq \Grad(\bN_u^e(\bm{X}))$ and $\bB_{0\Dbar}^e \coloneqq \Grad(\bN_{\Dbar}^e(\bm{X}))$ containing the derivatives of the element shape functions. Lastly, the Green-Lagrange strain increment $\D \bE$ and its corresponding test function $\delta \bE$ are approximated in terms of $\D \bm{u}^e$ and $\delta \bm{u}^e$:
\be
\D \bE(\bm{X}) \approx \mathbf{G}_{0u}^e(\bm{X}) \D \bm{u}^e \qquad \delta \bE(\bm{X}) \approx \mathbf{G}_{0u}^e(\bm{X}) \delta \bm{u}^e \qquad \bm{X} \in B_0^e
\ee
In the above equation, $\mathbf{G}_{0u}^e$ is a matrix containing products of the derivatives of the shape functions with components of the deformation gradient $\bF$. For further details regarding the finite element discretization, the interested reader is kindly referred to de Borst et al. \cite{NFEA} and Wriggers \cite{NFEM}.
Plugging the finite element approximations into equations \ref{eq:linmomentum} and \ref{eq:linmicromorphic} and introducing Voigt notation (also described in the literature mentioned above) for all tensors, one arrives at the following equations:
\bega
\sum_{e=1}^{n_{e l}} \delta \bm{u}^{e \top}\biggl\{\biggl(\underbrace{\int_{B_0^e} \mathbf{B}_{0 u}^{e \top} \mathcal{D}^e \mathbf{B}_{0 u}^e \mathrm{~d} V+\int_{B_0^e} \mathbf{G}_{0 u}^{e \top}\left(\frac{\partial \widehat{\mathbf{S}}}{\partial \widehat{\mathbf{E}}}\right)^e \mathbf{G}_{0 u}^e \mathrm{~d} V}_{:=\mathbf{k}_{u \mathrm{u}}^e}\biggr) \Delta \bm{u}^e\\+\underbrace{\int_{B_0^e} \mathbf{G}_{0 u}^{e \top}\left(\frac{\partial \widehat{\mathbf{S}}}{\partial \bar{D}}\right)^e \bN_{\bar{D}}^e \bar{\mathrm{d}} V}_{:=\mathbf{k}_{u \bar{D}}^e} \Delta^e \bar{\bm{D}}^e\biggr\} \\
=-\sum_{e=1}^{n_{\mathrm{el}}} \delta \bm{u}^{e \top}\biggl\{\underbrace{\int_{B_0^c} \mathbf{G}_{0 u}^{e \top} \widehat{\mathbf{S}}^e \mathrm{~d} V}_{:=\bm{r}_u^e}\underbrace{-\int_{B_0^e} \bN_u^{e \top} \mathbf{f}_0 \mathrm{~d} V-\int_{\partial B_{0 \mathrm{t}}^e} \bN_u^{e \top} \mathbf{t}_0 \mathrm{~d} A}_{:=\bm{p}_u^e}\biggr\}
\eega

\bega
\sum_{e=1}^{n_{\mathrm{cl}}} \delta \bar{\bm{D}}^{e \top}\biggl\{\underbrace{\int_{B_0^e} H \bN_{\bar{D}}^{e \top}\left(\frac{\partial D}{\partial \widehat{\mathbf{E}}}\right)^{e \top} \mathbf{G}_{0 u}^e \mathrm{~d} V}_{:=\mathbf{k}_{\bar{D} u}^e} \Delta \bm{u}^e\\
+\biggl(\underbrace{\int_{B_0^e} H\left(\left(\frac{\partial D}{\partial \bar{D}}\right)^e-1\right) \bN_{\bar{D}}^{e \top} \bN_{\bar{D}}^e \mathrm{~d} V-\int_{B_0^e} A \mathbf{B}_{0 \bar{D}}^{e \top} \mathbf{B}_{0 \bar{D}}^e \mathrm{~d} V}_{:=\mathbf{k}_{\bar{D}}^e}\biggr) \Delta \bar{\bm{D}}^e\biggr\} \\
=-\sum_{e=1}^{n_{\mathrm{cl}}} \delta \bar{\bm{D}}^{e \top}\biggl\{\underbrace{\int_{B_0^e} H \bN_{\bar{D}}^{e \top}\left(D^e-\bN_{\bar{D}}^e \bar{\bm{D}}^e\right) \mathrm{d} V-\int_{B_0^e} A \mathbf{B}_{0 \bar{D}}^{e \top} \mathbf{B}_{0 \bar{D}}^e \bar{\bm{D}}^e \mathrm{~d} V}_{:=\bm{r}_{\bar{D}}^e}\biggr\}
\eega
The introduced abbreviations $\mathbf{k}_{u u}^e$, $\mathbf{k}_{u \bar{D}}^e$, $\mathbf{k}_{\bar{D} u}^e$, $\mathbf{k}_{\bar{D} \bar{D}}^e$, $\bm{r}_{u}^e$, $\bm{p}_{u}^e$, $\bm{r}_{\bar{D}}^e$ are representing the different parts of the element stiffness matrix and the element residual vector. The terms $\D \bm{u}^e$ and $\D \bDbar^e$ are the nodal increments of the displacement and micromorphic damage. Assembling all element stiffness matrices via the finite element assembly operator $\asmbly(\bullet)$ yields the global matrices
\bega
\mathbf{K}_{uu} = \asmbly(\mathbf{k}_{u u}^e), \quad \mathbf{K}_{u\Dbar} = \asmbly(\mathbf{k}_{u \Dbar}^e), \quad \mathbf{K}_{\Dbar u} = \asmbly(\mathbf{k}_{\Dbar u}^e), \quad \mathbf{K}_{\Dbar \Dbar} = \asmbly(\mathbf{k}_{\Dbar \Dbar}^e)\\
\bR_{u} = \asmbly(\bm{r}_{u}^e), \quad \bP_{u} = \asmbly(\bm{p}_{u}^e), \quad \bR_{\Dbar} = \asmbly(\bm{r}_{\Dbar}^e)
\eega
Considering the boundary conditions as well as the fact that $\delta \bm{u}$ and $\delta \bDbar$ can be arbitrarily chosen and therefore neglected the global system of linear equations finally reads
\be
\underbrace{\left[\begin{array}{l l} \mathbf{K}_{uu} & \mathbf{K}_{u \Dbar}     \\
            \mathbf{K}_{\Dbar u}  & \mathbf{K}_{\Dbar \Dbar}
        \end{array} \right]}_{\mathbf{K}_T}
\underbrace{\left \{\begin{array}{l} \D \bm{u} \\
        \D \bDbar
    \end{array} \right \}}_{\D \bU}
= -
\underbrace{\left \{ \begin{array}{l} \bR_u + \bP_u \\
        \bR_{\Dbar}
    \end{array} \right \}}_{\bG}
\label{eq:soe}
\ee
The abbreviations $\mathbf{K}_T$ for the tangential stiffness matrix, $\D \bU$ for the incremental unknowns vector, and $\bG$ for the residual vector are introduced for later purposes. To get a solution to the problem at hand, the equation system \ref{eq:soe} is solved iteratively until convergence is achieved.
For further details regarding the equations and algorithmic implementation at the Gauss point level as well as a general study on the influence of the material parameters the work of Brepols et al. \cite{brepols2017, brepols2020} is highly recommended.
Because of the complexity of the material model, the computation of the stiffness matrix is fairly expensive. It should be noted at this point that in the present work, solely linear interpolation functions with 8 integration points per element are used. For completeness, the work of Barfusz et al. \cite{barfusz2021} should be highlighted, in which a single Gauss point formulation was implemented for the material model at hand and it was validated that the reduced integration approach still yields accurate results and can be used to increase the efficiency.

==> Chapter/2_Material_model_short.tex <==
\section{Material Model}
\label{sec:mat}


The aim of this publication is the demonstratoin of the possibilities and limitations of model order reduction. For this purpose, a gradient-extended two-surface damage plasticity model developed by Brepols et al. \cite{brepols2017, brepols2020} was chosen. Detailed equations and explanations can be found in their works. Here, only the essential equations will be briefly presented.
Under the assumption of linear kinematics, the strain is defined as the symmetric component of the displacement gradient. To model the behavior of elasto-plastic materials, the total strain is additively decomposed into elastic and plastic components. For nonlinear Armstrong-Frederick type kinematic hardening, an additional additive division of the plastic strain into recoverable and irrecoverable parts is used, expressed as
\be
\bvarepsilon = \bvarepsilon_{el}+\bvarepsilon_{p} = \bvarepsilon_{el}+\bvarepsilon_{p_e} + \bvarepsilon_{p_i}.
\ee

The Helmholtz free energy $\psi$ is assumed to follow an additive format:
\be
\psi = f_{\textrm{dam}}(D)(\psi_{el}(\bvarepsilon_{el})+\psi_p(\bvarepsilon_{p_e}, \xi_p))+\psi_d(\xi_d) + \psi_{\bar{d}}(D-\Dbar, \Grad(\Dbar))
\ee

where $\psi_{el}$ represents the elastic part and $\psi_p$ denotes the plastic part of the free energy. The plastic part is defined in terms of $\bvarepsilon_{p_e}$ and the isotropic hardening variable $ \xi_p$. The energy associated with damage hardening is stored in $\psi_d$, which depends on the damage hardening variable $\xi_d$. Furthermore, the contribution of the micromorphic extension is stored in $\psi_{\bar{d}}$, a function of the difference between the local damage variable $D$ and the micromorphic (or non-local) damage variable $\Dbar$, as well as its gradient $\Grad(\Dbar)$.
Furthermore, it is postulated that the degradation function $f_{\textrm{dam}}(D)$ with scalar values influences both the elastic and plastic energies.

Brepols et al. defined the elastic contribution $\psi_{el}$ as
\be
\psi_{el} \coloneqq \frac{1}{2}\bvarepsilon_{el} \cdot\mathbf{\mathcal{C}} \left[\bvarepsilon_{el}\right]
\ee


In the given expression, the variable $\mathbf{\mathcal{C}} \coloneqq \lambda \bm{I} \bigotimes \bm{I} + 2 \mu \mathbf{\mathcal{I}}$ symbolizes the isotropic fourth-order elasticity tensor, which combines the Lame constants $\lambda$, $\mu$, the second-order identity tensor $\bm{I}$ and the symmetric fourth-order identity tensor $\mathbf{\mathcal{I}}$ in its formulation. The plastic contribution 
\be
\psi_{p} \coloneqq \frac{1}{2} a \bvarepsilon_{p_e} \cdot \bvarepsilon_{p_e} + e \left( \xi_p + \frac{\exp ( -f \xi_p) -1}{f}   \right)
\ee
contains the material parameters $a$, $e$ and $f$. These are related to kinematic and non-linear Voce isotropic hardening. 
\be
\psi_{d} \coloneqq r \left( \xi_d + \frac{\exp(-s\xi_d)-1}{s} \right)
\ee
is defined to model the non-linear Voce damage hardening. This expression contains the parameters $r$ and $s$.
The term of the Helmholtz free energy which is related to the micromorphic extension of the model is defined by
\be
\psi_{\bar{d}} \coloneqq \frac{1}{2} H \left( D- \Dbar \right)^2 + \frac{1}{2} A \Grad (\Dbar) \cdot \Grad (\Dbar).
\ee
A strong coupling between the local and the micromorphic damage variable is allowed through the penalty parameter $H$, which is usually chosen as a very high number. The parameter $A$ controlls the influence of the gradient $\bar{D}$. 
An internal length scale is introduced with the quotient
\be
L \coloneqq \sqrt{\frac{A}{H}}.
\ee
The internal length $L$ is required to limit the localization and prevents that the damage zone shrinks into a single row of elements.  The constitutive equations with respect to the reference configuration are based on the Clausius-Duhem inequality in order to fulfill the second law of thermodynamics. The derivation of the constitutive equations is carefully described by Brepols et al. \cite{brepols2020} and, because it is not the main topic of this thesis, only the resulting equations are given below:

\begin{itemize}
    \item State laws:
        \bea
        \bS &= \fdam(D) \, 2 \, \bF_p\ME \dfrac{\partial \psi_e}{\partial \bC_e}\bF_p\MT\\
        &= \fdam(D) \left(\mu \, (\bC_p\ME - \bC\ME) + \dfrac{\lambda}{2} \left(\dfrac{\det \bC}{\det \bC_p} - 1 \right) \bC\ME \right)
        \eea
    \item Thermodynamic conjugate forces - plasticity 
        \be
        \bX = \fdam(D) \, 2 \, \bF_{p_i}\ME \dfrac{\partial \psi_e}{\partial \bC_{p_e}}\bF_{p_i}\MT = \fdam(D)\,a\,(\bC_{p_i}\ME - \bC\ME)
        \ee
        \be
        q_p = \fdam(D)\,\dfrac{\partial \psi_p}{\partial \xi_p} = \fdam(D)\,e\,(1 - \exp(-f\xi_p))
        \ee

    \item Thermodynamic conjugate forces - damage (driving force Y and damage hardening $q_d$):
        \be
        Y = - \dfrac{\dd \fdam(D)}{\dd D}\,(\psi_e+\psi_p)-\dfrac{\partial \psi_{\bar{d}}}{\partial D} = - \dfrac{\dd \fdam(D)}{\dd D}\,(\psi_e+\psi_p) - H(D-\Dbar)
        \ee
        \be
        q_d = \dfrac{\partial \psi_d}{\partial \xi_d} = r\,(1 - \exp(-s \, \xi_d))
        \ee
    \item Auxillary stress tensors:
        \be
        \bY = \bC \bS - \bC_p \bX, \quad \bY_{\textrm{kin}} = \bC_p \bX
        \ee
    \item Evolution equations with a constant additional plastic material parameter $b$ to model non-linear kinematic hardening :
        \be
        \dot{\bC}_p = 2 \, \dot{\lambda}_p \dfrac{\sqrt{3/2}}{\fdam(D)}\dfrac{\tilde{\bY}^{'} \bC_p}{\sqrt{\tilde{\bY}^{'} \cdot (\tilde{\bY}^{'})\T}}, \quad \dot{\bC}_{p_i} = 2 \, \dot{\lambda}_p \dfrac{b/a}{\fdam(D)} \bY^{'}_{\textrm{kin}} \bC_{p_i}
        \ee
        \be
        \dot{\xi}_p = \dfrac{\dot{\lambda}_p}{\fdam(D)}, \quad \dot{D} = \dot{\lambda}_d, \quad \dot{\xi}_d = \dot{\lambda}_d
        \ee
    \item Yield and damage loading function where $\sigma_0$ and $Y_0$ represents the initial yield stress and the damage threshold:
        \be
        \Phi_p = \sqrt{3/2} \sqrt{\tilde{\bY}^{'} \cdot (\tilde{\bY}^{'})\T} - (\sigma_0 + \tilde{q}_p), \quad \Phi_d = Y - (Y_0 + q_d)
        \label{eq:threshold}
        \ee
    \item Loading / unloading conditions
        \bea
        \dot{\lambda}_p \ge 0, \qquad \Phi_p \le 0, \qquad \dot{\lambda}_p \Phi_p = 0\\
        \dot{\lambda}_d \ge 0, \qquad \Phi_d \le 0, \qquad \dot{\lambda}_d \Phi_d = 0
        \eea
\end{itemize}

Overall, the material possesses twelve distinct material parameters ($\lambda$, $\mu$, $\sigma_0$, $a$, $b$, $e$, $f$, $Y_0$, $r$, $s$, $H$, $A$) that need to be determined experimentally. However, this aspect is beyond the scope of this publication and will be selected subsequently. The corresponding system of nonlinear equations can be solved using the Newton-Raphson scheme. Further details regarding the material model can be found in Brepols et al. \cite{brepols2020}.
